Joint-Task Regularization for Partially Labeled Multi-Task Learning

Multi-task learning has become increasingly popular in the machine learning field, but its practicality is hindered by the need for large, labeled datasets. Most multi-task learning methods depend on fully labeled datasets wherein each input example is accompanied by ground-truth labels for all target tasks. Unfortunately, curating such datasets can be prohibitively expensive and impractical, especially for dense prediction tasks which require per-pixel labels for each image. With this in mind, we propose Joint-Task Regularization (JTR), an intuitive technique which leverages cross-task relations to simultaneously regularize all tasks in a single joint-task latent space to improve learning when data is not fully labeled for all tasks. JTR stands out from existing approaches in that it regularizes all tasks jointly rather than separately in pairs -- therefore, it achieves linear complexity relative to the number of tasks while previous methods scale quadratically. To demonstrate the validity of our approach, we extensively benchmark our method across a wide variety of partially labeled scenarios based on NYU-v2, Cityscapes, and Taskonomy.

==> table/fig_xtr_training.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{figure/fig:xtr_img.pdf} %
    \caption{
        Visualizations for an input image from NYUv2, its corresponding ground truth labels, the model's predictions, JLR's intermediate joint-task space representations, a heatmap of the JLR loss term using cosine similarity, and the final reconstructed predictions/labels. Here, $\mathcal{L}_{Recon}$ prevents the joint-task representations from collapsing to a trivial solution, and $\mathcal{L}_{JLR}$ guides the unlabeled tasks by enforcing consistency with available labels in the joint-task space. 
        %
        %
        %
        %
        %
        %
        %
        %
        }
    \label{fig:xtr_training}
\end{figure}

==> table/tab_resource_taskonomy.tex <==
\begin{table}[t]
    \centering
    \tablescale{
    {
		\begin{tabular}{lccccc}
            \toprule
            \multirow{2}{*}{Method}  & \multicolumn{4}{c}{Taskonomy} \\
            & Data $\downarrow$ & model $\downarrow$ & Step $\downarrow$ & t-step $\downarrow$ & VRAM $\downarrow$\\
            \midrule
            Supervised MTL & 0.202 & 0.134 & 0.450 & 0.410 (0.025) & 9904MB \\ %
            x32468 (6815) & 1h50m & 1h13m & 4h4m & 47m & 4h51m \\
            Consistency Reg. & 0.197 & 0.145 & 0.450 & 0.415 (0.041) & 10184MB \\
            x32468 (6815)  &  1h47m  &  1h18m  & 4h4m & 47m   &   4h51m \\
            MTPSL \cite{li2022learning}& 0.020 & 1.029 & 1.152 & 0.410 (0.025) & 34396MB \\
            x32468 (6815)  &   11m &  9h17m  & 10h23m & 47m & 11h10m \\
            \textbf{Ours (JTR)} & 0.020 & 0.375 & 0.495 & 0.403 (0.025) &  23952MB\\
            x32468 (6815) & 11m  & 3h23m & 4h28m  & 47m & 5h15m \\
            %
            %
            %
            %
            %
            %
            %
            \bottomrule
		\end{tabular}
    }
    }
    \caption{
        \textcolor{red}{This table is just for archiving.
        This table will be removed.}
        Time and VRAM requirements for training each method using the SegNet architecture on Taskonomy on an NVIDIA A100, with batch sizes $8$.
        (js: Taskonomy resource measured by NVIDIA A100-SXM4-80GB. Per epoch resource calculation.)
    }
    %
    \label{tab:generalperf}
\end{table}

==> table/tab_ssl_all.tex <==
\begin{table}[t]
    \centering
    \resizebox{1.0\textwidth}{!}{
            \setlength{\tabcolsep}{6pt}
		\begin{tabular}{clcccc@{\hskip 0.4in}ccc}
            \toprule
            \multirow{2}{*}{Label Scenario} & \multirow{2}{*}{Method} & \multicolumn{4}{c}{NYU-v2} \hspace{10mm}& \multicolumn{3}{c}{Cityscapes}\hspace{6mm}\\
            %
            & & Seg. $\uparrow$ & Depth $\downarrow$ & Norm. $\downarrow$ & $\Delta$MTL (\%) $\uparrow$ & Seg. $\uparrow$ & Depth $\downarrow$ & $\Delta$Avg$\%$ $\uparrow$ \\
            \midrule
            \multirow{1}{*}{full} 
            & Supervised Learning           & 38.91 & 0.5351 & 28.57 & +0.000   & 73.36 & 0.0165 & +0.000  \\
            \midrule
            %
            %
            \multirow{4}{*}{\shortstack[c]{70\% random, \\ 30\% unlabeled}}
            & Supervised Learning           & 26.36 & 0.6574 & 33.02 & +0.000   & 69.62 & 0.0180 & +0.000 \\
            & Consistency Regularization    & 29.89 & 0.6136 & 31.93 & +7.777   & 69.65 & 0.0171 & +2.522 \\
            %
            & MTPSL \cite{li2022learning}                         & 31.92 & 0.6071 & 31.59 & +11.02   & \textbf{71.48} & 0.0169 & +4.391 \\
            %
            %
            %
            %
            \cmidrule{2-9}
            & \textbf{Ours (XTR)}           & \textbf{32.20} & \textbf{0.5912} & \textbf{31.01} & \textbf{+12.78} & 71.07 & \textbf{0.0161} & \textbf{+6.319}\\
            %
            \midrule
            %
            %
            \multirow{4}{*}{\shortstack[c]{50\% random, \\ 50\% unlabeled}} 
            & Supervised Learning           & 23.68 & 0.6988 & 35.00 & +0.000   & 67.56 & 0.0196 & +0.000 \\
            & Consistency Regularization    & 25.16 & 0.6543 & 32.54 & +6.548   & 69.23 & 0.0174 & +6.848 \\
            & MTPSL \cite{li2022learning}                         & 28.18 & 0.6393 & 33.04 & +11.04   & \textbf{70.30} & 0.0174 & +7.640\\
            %
            \cmidrule{2-9}
            %
            & \textbf{Ours (XTR)} & {\bf 28.69} & \textbf{0.6268} & \textbf{31.52} & \textbf{+13.81} & 69.76 & \textbf{0.0167} & \textbf{+9.026}\\
            %
            \midrule
            %
            %
            \multirow{4}{*}{\shortstack[c]{30\% random, \\ 70\% unlabeled}} 
            & Supervised Learning           & 18.57 & 0.7288 & 37.49 & +0.000   & 64.65 & 0.0217 & +0.000 \\
            & Consistency Regularization    & 20.60 & 0.7135 & 34.81 & +6.723   & 66.43 & 0.0187 & +8.289 \\
            & MTPSL \cite{li2022learning}                         & 23.33 & 0.6952 & 34.81 & +12.47   & \textbf{68.09} & 0.0187 & +9.573 \\
            %
            %
            %
            \cmidrule{2-9}
            %
            & \textbf{Ours (XTR)}           & \textbf{24.05} & \textbf{0.6945} & \textbf{34.25} & \textbf{+14.30} & 67.75 & \textbf{0.0179} & \textbf{+11.15} \\
             %
            \bottomrule
		\end{tabular}
    }
    \vspace{0.5em}
    \caption{Semi-supervised partially labeled multi-task learning results on NYU-v2 and Cityscapes. RandAugment \cite{cubuk2020randaugment} is used for all experiments. The distributions of labels for the labeled portions of the dataset are kept consistent with the ``random'' label scenario from Tab. \ref{tab:nyuv2}.}
    \label{tab:ssl_all}
    %
    %
\end{table}

==> table/tab_ssl_cityscapes.tex <==
\begin{table}
    \centering
    \tablescale{
		\begin{tabular}{lccc}
            \toprule
            Method & Seg. $\uparrow$ & Depth $\downarrow$ & $\Delta$Avg$\%$ $\uparrow$ \\
            \midrule
            %
            %
            %
            %
            %
            \multicolumn{4}{c}{\textit{70\% randomlabels, 30\% unlabeled}}\\
            Supervised Learning           & 69.62 & 0.0180 &  +0.000\\
            Consistency Reg. (SSL)    & 69.65 & 0.0171 &  \\
            MTPSL~\cite{li2022learning}                         & \textbf{71.48} & 0.0169 &  \\
            %
            %
            \cmidrule{1-4}
            \textbf{Ours (XTR)}           & 71.07 & \textbf{0.0161} & \textbf{}\\
            \midrule
            %
            %
            \multicolumn{4}{c}{\textit{50\% randomlabels, 50\% unlabeled}}\\
            Supervised Learning           & 67.56 & 0.0196 & +0.000\\
            Consistency Reg. (SSL)    & 69.23 & 0.0174 & \\
            MTPSL~\cite{li2022learning}                         & \textbf{70.30} & 0.0174 & \\
            %
            %
            %
            %
            \cmidrule{1-4}
            \textbf{Ours (XTR)}           & 69.76 & \textbf{0.0167} & \textbf{}\\
            \midrule
            %
            %
            \multicolumn{4}{c}{\textit{30\% randomlabels, 70\% unlabeled}}\\
            Supervised Learning           & 64.65 & 0.0217 & 0.000 \\
            Consistency Reg. (SSL)    & 66.43 & 0.0187 &  \\
            MTPSL~\cite{li2022learning} & \textbf{68.09} & 0.0187 &  \\
            %
            %
            %
            %
            %
            \cmidrule{1-4}
            \textbf{Ours (XTR)}        & 67.75 & \textbf{0.0179} & \textbf{}\\
            \bottomrule
		\end{tabular}
    }
    \vspace{0.5em}
    \caption{Semi-supervised partially labeled multi-task learning results on Cityscapes. RandAugment~\cite{cubuk2020randaugment} is used for all experiments. The distributions of labels for the labeled portions of the dataset are kept consistent with the ``one'' label scenario from Tab. \ref{tab:cityscapes}.}
    \label{tab:ssl_cityscapes}
    \vspace{-0.5em}
\end{table}

==> table/tab_taskonomy_limit1000.tex <==
% 
%
\begin{table*}
    \centering
    \tablescale{{
		\begin{tabular}{llccccccc a}%
            \toprule
            Scenario & Method & $\Delta$Seg.$\%$  & $\Delta$Depth$\%$ & $\Delta$Norm.$\%$ &
            $\Delta$Occl.$\%$ & $\Delta$Resh.$\%$ & $\Delta$KeyP.$\%$ & $\Delta$Text.$\%$ &
            $\overbar{\Delta\%}$ $\uparrow$
            %
            \\
            \midrule
            %
            %
            %
            %
            %
            %
            \multirow{3}{*}{\textit{onelabel}}& Consistency Reg.            & -0.2509 & +1.288 & +19.30 & -0.641 & -2.950 & +12.28 & +14.55 & +2.482 \\
            & MTPSL \cite{li2022learning} & +0.3557 & +5.638 & +23.57 & +1.121 & +3.455 & +7.542 & +25.12 & +4.240 \\ 
            & \textbf{Ours (JTR)}         & +0.1565 & +3.770 & +24.61 & +0.648 & +1.524 & +13.15 & +35.09 & \textbf{+4.870} \\
            \midrule
            %
            %
            %
            \multirow{3}{*}{\textit{randomlabels}}& Consistency Reg.            & -0.645 & -6.332 & +25.01 & -0.502 & -4.683 & +9.110 & +20.85 & +2.676 \\
            & MTPSL \cite{li2022learning} & +0.022 & +5.716 & +30.50 & +1.936 & +5.375 & +16.56 & +31.35 & +5.716 \\
            & \textbf{Ours (JTR)}         & +0.015 & +1.942 & +32.41 & +2.270 & +3.309 & +19.96 & +41.62 & \textbf{+6.345}\\
            \midrule
            %
            %
            %
            \multirow{3}{*}{\textit{halflabels}} & Consistency Reg.            & -0.818 & -5.528 & +19.27 & +0.207 & -4.409 & +23.28 & +22.47 & +3.405 \\
            & MTPSL \cite{li2022learning} & -0.080 & +4.868 & +23.24 & +1.730 & +6.065 & +6.631 & +28.79 & +4.453 \\
            & \textbf{Ours (JTR)}         & -0.511 & +0.186 & +20.39 & +0.815 & +1.250 & +14.63 & +40.56 & {\bf+4.832}  \\ 
            %
            \bottomrule
		\end{tabular}
    }}
    %
    \caption{Partially labeled MTL results on Taskonomy. Scores are relative percentage improvements over the ``Supervised MTL'' baseline.}
    \label{tab:taskonomy}
    \vspace{-0.5em}
    %
\end{table*}

==> table/tab_taskonomy_v1.tex <==
%
\begin{table}
    \centering
    \tablescale{{
		\begin{tabular}{lcc@{\hskip 2em}cc}
            \toprule
            Method & $\Delta$Loss $\uparrow$ & $\overbar{\Delta\%}$ $\uparrow$ 
            & $\Delta$Loss $\uparrow$ & $\overbar{\Delta\%}$ $\uparrow$ \\
            \midrule
            & \multicolumn{2}{c}{\textit{all}} & \multicolumn{2}{c}{\textit{subset}}\\
            \cmidrule(lr){2-5}
            %
            %
            %
            %
            & \multicolumn{4}{c}{\textit{onelabel}}\\
            Supervised MTL & +0.000 & +0.000 & +0.000 & +0.000 \\
            Consistency Reg. & -2.363 & -1.401 & +1.288 & +2.482 \\
            MTPSL \cite{li2022learning}& +0.103 & +0.007 & +5.253 & +4.240 \\ 
            \textbf{Ours (JTR)}& +3.164 & \textbf{+4.917} & +5.238 & \textbf{+4.870} \\
            %
            %
            & \multicolumn{4}{c}{\textit{randomlabels}}\\
            Supervised MTL & +0.000 & +0.000 & +0.000 & +0.000 \\
            Consistency Reg. & -1.447 & -0.620 & -1.667 & +2.676 \\
            MTPSL \cite{li2022learning} & +0.513 & -0.156 & +5.681 & +5.716 \\
            \textbf{Ours (JTR)} & +2.360 & \textbf{+2.859} & +3.257 & \textbf{+5.810} \\
            \midrule
            %
            & \multicolumn{4}{c}{\textit{halflabels}}\\
            Supervised MTL & +0.000 & +0.000 & +0.000 & +0.000 \\
            Consistency Reg. & -3.207 & -0.343 & -2.345 & +3.405 \\
            MTPSL \cite{li2022learning}& -1.513 & -0.767 & +3.873 & +4.453 \\
            \textbf{Ours (JTR)} & +1.882 & {\bf +3.063} &  +1.899 & {\bf +4.823}  \\ 
            %
            \bottomrule
		\end{tabular}
    }}
    %
    \caption{Partially labeled multi-task learning results on Taskonomy. (Results from Nov-15 2:14AM)}
    \label{tab:taskonomy}
    \vspace{-1em}
    %
\end{table}

==> utils/custom.tex <==
% %
%
\usepackage{xspace}
\usepackage{amsmath,amssymb}
\usepackage[normalem]{ulem}
\usepackage{xcolor,colortbl}

\makeatletter
\def\onedot{\ifx\@let@token.\else.\null\fi\xspace}
\makeatother
%


\makeatletter
\newcommand*\bigcdot{\mathpalette\bigcdot@{.5}}
\newcommand*\bigcdot@[2]{\mathbin{\vcenter{\hbox{\scalebox{#2}{$\m@th#1\bullet$}}}}}
\makeatother

\def\eg{\textit{e.g}\onedot} \def\Eg{{E.g}\onedot}
\def\ie{\textit{i.e}\onedot} \def\Ie{{I.e}\onedot}
\def\cf{\textit{c.f}\onedot} \def\Cf{{C.f}\onedot}
\def\etc{\textit{etc}\onedot} \def\vs{{vs}\onedot}
\def\wrt{\textit{w.r.t}\onedot} \def\dof{d.o.f\onedot}
\def\etal{\textit{et al}\onedot}
\def\lowcomma{_{\textstyle,}}



\newcommand{\Tref}[1]{Tab.~\ref{#1}}
\newcommand{\Eref}[1]{Eq.~(\ref{#1})}
\newcommand{\Fref}[1]{Fig.~\ref{#1}}
\newcommand{\FCref}[1]{Chapter.~\ref{#1}}
\newcommand{\Cref}[1]{Chap.~\ref{#1}}
\newcommand{\Sref}[1]{Sec.~\ref{#1}}
\newcommand{\Aref}[1]{Alg.~\ref{#1}}

\newcommand{\R}{\mathbb{R}}
\newcommand{\matL}{\mathbf{Z}}
\newcommand{\matS}{\mathbf{E}}
\newcommand{\X}{\mathbf{X}}
\newcommand{\Y}{\mathbf{Y}}
\newcommand{\I}{\mathbf{I}}
\newcommand{\Z}{\mathbf{Z}}

\newcommand{\CovX}{\mathbf{\Phi}}
\newcommand{\CovS}{\mathbf{\Gamma}}

\newcommand{\D}{\mathbf{D}}
\newcommand{\singularmat}{\Sigma}




\def\Vec#1{\mbox{\boldmath $#1$}}
\newcommand{\mO}{\mathbf{O}}
\newcommand{\mc}{\mathbf{c}}

\newcommand{\paragrp}[1]{\vspace{1mm}\noindent\textbf{#1}\,\,\,}

%
\definecolor{steelblue}{rgb}{0.27, 0.51, 0.7}
\newcommand{\js}[1]{\textcolor{steelblue}{#1}}
\newcommand{\wl}[1]{\textcolor{purple}{WL: #1}}
\newcommand{\overbar}[1]{\mkern 1.5mu\overline{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu}
\newcommand{\tablescale}[1]{{\scalebox{0.85}{#1}}}
\setlength\tabcolsep{5pt}



\definecolor{Gray}{gray}{0.90}
\newcolumntype{a}{>{\columncolor{Gray}}c}
